Deception in Supervisory Control

The use of deceptive strategies is important for an agent that attempts not to reveal his intentions in an adversarial environment. We consider a setting in which a supervisor provides a reference policy and expects an agent to follow the reference policy and perform a task. The agent may instead follow a different, deceptive policy to achieve a different task. We model the environment and the behavior of the agent with a Markov decision process, represent the tasks of the agent and the supervisor with reachability specifications, and study the synthesis of optimal deceptive policies for such agents. We also study the synthesis of optimal reference policies that prevent deceptive strategies of the agent and achieve the supervisor's task with high probability. We show that the synthesis of optimal deceptive policies has a convex optimization problem formulation, while the synthesis of optimal reference policies requires solving a nonconvex optimization problem. We also show that the synthesis of optimal reference policies is NP-hard.

==> images/restimessupTIKZ.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{1.00000,1.00000,0.00000}%
%
\begin{tikzpicture}

\begin{axis}[%
width=4.047in,
height=3.566in,
at={(0.679in,0.481in)},
scale only axis,
point meta min=0,
point meta max=1.8,
axis on top,
xmin=0,
xmax=21,
y dir=reverse,
ymin=0,
ymax=21,
axis line style={draw=none},
ticks=none,
legend style={legend cell align=left, align=left, draw=white!15!black},
colormap={mymap}{[1pt] rgb(0pt)=(0.9,0.9447,0.9741); rgb(63pt)=(0,0.447,0.741)},
colorbar
]
\addplot [forget plot] graphics [xmin=0.5, xmax=20.5, ymin=0.5, ymax=20.5] {restimessupTIKZ-1.png};
\draw[fill=mycolor1, draw=none] (axis cs:16.5,6.5) rectangle (axis cs:17.5,7.5);
\draw[fill=green, draw=none] (axis cs:3.5,12.5) rectangle (axis cs:4.5,13.5);
\draw[fill=red, draw=none] (axis cs:11.5,15.5) rectangle (axis cs:12.5,16.5);
\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	0.5\\
0.5	20.5\\
};
\addlegendentry{data1}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
1.5	0.5\\
1.5	20.5\\
};
\addlegendentry{data2}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
2.5	0.5\\
2.5	20.5\\
};
\addlegendentry{data3}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
3.5	0.5\\
3.5	20.5\\
};
\addlegendentry{data4}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
4.5	0.5\\
4.5	20.5\\
};
\addlegendentry{data5}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
5.5	0.5\\
5.5	20.5\\
};
\addlegendentry{data6}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
6.5	0.5\\
6.5	20.5\\
};
\addlegendentry{data7}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
7.5	0.5\\
7.5	20.5\\
};
\addlegendentry{data8}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
8.5	0.5\\
8.5	20.5\\
};
\addlegendentry{data9}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
9.5	0.5\\
9.5	20.5\\
};
\addlegendentry{data10}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
10.5	0.5\\
10.5	20.5\\
};
\addlegendentry{data11}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
11.5	0.5\\
11.5	20.5\\
};
\addlegendentry{data12}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
12.5	0.5\\
12.5	20.5\\
};
\addlegendentry{data13}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
13.5	0.5\\
13.5	20.5\\
};
\addlegendentry{data14}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
14.5	0.5\\
14.5	20.5\\
};
\addlegendentry{data15}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
15.5	0.5\\
15.5	20.5\\
};
\addlegendentry{data16}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
16.5	0.5\\
16.5	20.5\\
};
\addlegendentry{data17}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
17.5	0.5\\
17.5	20.5\\
};
\addlegendentry{data18}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
18.5	0.5\\
18.5	20.5\\
};
\addlegendentry{data19}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
19.5	0.5\\
19.5	20.5\\
};
\addlegendentry{data20}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
20.5	0.5\\
20.5	20.5\\
};
\addlegendentry{data21}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	0.5\\
20.5	0.5\\
};
\addlegendentry{data22}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	1.5\\
20.5	1.5\\
};
\addlegendentry{data23}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	2.5\\
20.5	2.5\\
};
\addlegendentry{data24}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	3.5\\
20.5	3.5\\
};
\addlegendentry{data25}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	4.5\\
20.5	4.5\\
};
\addlegendentry{data26}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	5.5\\
20.5	5.5\\
};
\addlegendentry{data27}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	6.5\\
20.5	6.5\\
};
\addlegendentry{data28}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	7.5\\
20.5	7.5\\
};
\addlegendentry{data29}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	8.5\\
20.5	8.5\\
};
\addlegendentry{data30}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	9.5\\
20.5	9.5\\
};
\addlegendentry{data31}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	10.5\\
20.5	10.5\\
};
\addlegendentry{data32}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	11.5\\
20.5	11.5\\
};
\addlegendentry{data33}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	12.5\\
20.5	12.5\\
};
\addlegendentry{data34}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	13.5\\
20.5	13.5\\
};
\addlegendentry{data35}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	14.5\\
20.5	14.5\\
};
\addlegendentry{data36}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	15.5\\
20.5	15.5\\
};
\addlegendentry{data37}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	16.5\\
20.5	16.5\\
};
\addlegendentry{data38}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	17.5\\
20.5	17.5\\
};
\addlegendentry{data39}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	18.5\\
20.5	18.5\\
};
\addlegendentry{data40}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	19.5\\
20.5	19.5\\
};
\addlegendentry{data41}

\addplot [color=white!70!black]
  table[row sep=crcr]{%
0.5	20.5\\
20.5	20.5\\
};
\addlegendentry{data42}

\end{axis}
\end{tikzpicture}%
